Sparse Autoencoders Find Highly Interpretable Features in Language Models

One of the roadblocks to a better understanding of neural networks' internals is \textit{polysemanticity}, where neurons appear to activate in multiple, semantically distinct contexts. Polysemanticity prevents us from identifying concise, human-understandable explanations for what neural networks are doing internally. One hypothesised cause of polysemanticity is \textit{superposition}, where neural networks represent more features than they have neurons by assigning features to an overcomplete set of directions in activation space, rather than to individual neurons. Here, we attempt to identify those directions, using sparse autoencoders to reconstruct the internal activations of a language model. These autoencoders learn sets of sparsely activating features that are more interpretable and monosemantic than directions identified by alternative approaches, where interpretability is measured by automated methods. Moreover, we show that with our learned set of features, we can pinpoint the features that are causally responsible for counterfactual behaviour on the indirect object identification task \citep{wang2022interpretability} to a finer degree than previous decompositions. This work indicates that it is possible to resolve superposition in language models using a scalable, unsupervised method. Our method may serve as a foundation for future mechanistic interpretability work, which we hope will enable greater model transparency and steerability.

==> neurips_workshop/autointerp_neurips.tex <==
We assess our interpretability scores against a variety of alternative methods for finding dictionaries of features in language models. In particular, we compare interpretability scores on our dictionary features to those produced by a) the default basis, b) random directions, c) Principal Component Analysis (PCA), and d) Independent Component Analysis (ICA). For the random directions and for the default basis in the residual stream, we replace negative activations with zeros so that all feature activations are nonnegative \footnote{
For PCA we use an online estimation approach and run the decomposition on the same quantity of data we used for training the autoencoders. For ICA, due to the slower convergence times, we run on only 2GB of data, approximately 4 million activations for the residual stream and 1m activations for the MLPs.}.

% Sparse coding differs significantly to the aforementioned baselines in that it has a bias and then a ReLU applied to the direction which allows it to be sensitive to smaller regions of the activation space. This removes some of the noise from the activations which could make it easier to predict a high proportion of the variance. To ensure we are comparing to fair baselines, we create Top-K versions of PCA and ICA in which only the top K directions most relevant to a given datapoint are retained, and the rest are set to zero. We select K to match the average number of features active per token for the learned dictionary with ratio 1 and l1 $\alpha$ of 8e-4.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{images/residual_top_random_means_and_cis_new.png}
    \caption{Average top-and-random autointerpretability score of  our learned directions in the residual stream, compared to a number of baselines, using 150 features each. Error bars show 95\% confidence intervals around means. The feature dictionaries used here were trained for 10 epochs using $\alpha=.00086$ and $R=2$.}
    \label{fig:main_interp_scores_comparison}
\end{figure}


Figure \ref{fig:main_interp_scores_comparison} shows that our dictionary features are far more interpretable by this measure than dictionary features found by comparable techniques. We find that the strength of this effect declines as we move through the model, being comparable to ICA in layer 4 and showing minimal improvement in the final layer.

This could indicate that sparse autoencoders work less well in later layers but also may be connected to the difficulties of automatic interpretation, both because by building on earlier layers, later features may be more complex, and because they are often best explained by their effect on the output. \citet{bills2023language} showed that GPT-4 is able to generate explanations that are very close to the average quality of the human-generated explanations given similar data. However, they also showed that current LLMs are limited in the kinds of patterns that they can find, sometimes struggling to find patterns that center around next or previous tokens rather than the current token, and in the current protocol are unable to verify outputs by looking at changes in output or other data. 


See Appendix \ref{appendix:full_autointerp} for a fuller exploration of different learned dictionaries through the lens of automatic interpretability, looking at both the MLPs and the residual stream.

==> neurips_workshop/dictionary_learning_neurips.tex <==
\label{section:sparse_autoencoder}
To take network features out of superposition, we employ techniques from \emph{sparse dictionary learning} \citep{olshausen1997sparse, lee2006efficient}. Suppose that each of a given set of vectors $\{\mathbf{x}_i\}_{i=1}^{n_{\text{vec}}} \subset \R^d$ is composed of a sparse linear combination of unknown vectors $\{\mathbf{g}_j\}_{j=1}^{n_{\text{gt}}} \subset \R^d$, i.e. $\mathbf{x}_i = \sum_j a_{i,j}\mathbf{g}_j$ where $\mathbf{a_i}$ is a sparse vector. In our case, the data vectors $\{\mathbf{x}_i\}_{i=1}^{n_{\text{vec}}}$ are internal activations of a language model, such as Pythia-70M \citep{biderman2023pythia}, and $\{\mathbf{g}_j\}_{j=1}^{n_{\text{gt}}}$ are unknown, ground truth network features. We would like learn a dictionary of vectors, called dictionary features, $\{\mathbf{f}_k\}_{k=1}^{n_{\text{feat}}} \subset \R^d$ where for any network feature $\mathbf{g}_j$ there exists a dictionary feature $\mathbf{f}_k$ such that $\mathbf{g}_j \approx \mathbf{f}_k$. 

%Using gradient descent to $\mathbf{x}_i \approx \sum_j c_{i,j}\mathbf{f}_j$
% find a dictionary of vectors, called dictionary features, $\{\mathbf{f}_j\}_{j=1}^{n_{\text{feat}}} \subset \R^d$ such that each of a given set of vectors $\{\mathbf{x}_i\}_{i=1}^{n_{\text{vec}}} \subset \R^d$ can be represented as a sparse linear combination of features $\mathbf{x}_i=\sum_j c_{i,j}\mathbf{f}_j$. It can be shown that linear combinations of ground truth features can be recovered by $\ell^1$ minimisation \citep{wright_ma_2022}. This is done by minimising the $\ell^1$ norm of the coefficients which acts as a proxy for minimising the number of active features while being more computationally tractable \citep{wright_ma_2022}.
%In our case, the data vectors $\{\mathbf{x}_i\} \subset \R^d$ are internal activations of a language model such as Pythia-70M \citep{biderman2023pythia}. Under the `linear with superposition' hypothesis,  we assume that the $\{\mathbf{x}_i\}$ are actually a linear combination of unknown, ground-truth network features, which we try to identify using sparse dictionary learning. 
%would form a sparse dictionary. We therefore expect that sparse dictionary learning will be able to learn a set of features $\{\mathbf{f}_j\}$ similar to the ground-truth features, while being human-understandable.
To learn the dictionary, we train an autoencoder with a sparsity penalty term on its hidden activations. The autoencoder is a neural network with a single hidden layer of size $d_{\text{hid}}=R d_{\text{in}}$, where $d_{\text{in}}$ is the dimension of the language model internal activation vectors\footnote{We mainly study residual streams in Pythia-70M and Pythia 410-M, for which the residual streams are of size $d_{\text{in}}=512$ and $d_{\text{in}}=1024$, respectively \citep{biderman2023pythia}}, and $R$ is a hyperparameter that controls the ratio of the feature dictionary size to the model dimension. We use the ReLU activation function in the hidden layer \citep{fukushima1975relu}. We also use tied weights for our neural network, meaning the weight matrices of the encoder and decoder are transposes of each other.\footnote{We use tied weights because (a) they encode our expectation that the directions which detect and define the feature should be the same or highly similar, (b) they halve the memory cost of the model, and 
(c) they remove ambiguity about whether the learned direction should be interpreted as the encoder or decoder direction. They do not reduce performance when training on residual stream data but we have observed some reductions in performance when using MLP data.}  Thus, on input vector $\mathbf{x} \in \{\mathbf{x}_i\}$, our network produces the output $\mathbf{\hat x}$, given by $\mathbf{c} = \mathrm{ReLU}(M\mathbf{x}+\mathbf{b})$ and $\mathbf{\hat x} = M^T \mathbf{c} \label{eq:decoder} =\displaystyle  \sum_{i = 0}^{d_{\text{hid}}-1} c_i \mathbf{f}_i$, where $M \in \R^{d_{\text{hid}} \times d_{\text{in}}}$ and $\mathbf{b} \in \R^{d_{\text{hid}}}$ are our learned parameters, and $M$ is normalised row-wise\footnote{Normalisation of the rows (dictionary features) prevents the model from reducing the sparsity loss term $||\mathbf{c}||_1$ by increasing the size of the feature vectors in $M$.}. Our parameter matrix $M$ is our feature dictionary, consisting of $d_{\text{hid}}$ rows of dictionary features $\mathbf{f}_i$. The output $\mathbf{\hat x}$ is meant to be a reconstruction of the original vector $\mathbf x$, and the hidden layer $\mathbf c$ consists of the coefficients we use in our reconstruction of $\mathbf x$. 


% In this architecture, the parameter matrix $M$ consists of the $d_{\text{hid}}$ feature vectors which we wish to train and interpret, 

% \begin{figure} \label{fig:Architecture}
% \includegraphics[width=0.9\textwidth]{images/Architecture v3.png}
% \caption{Architecture and loss function of our sparse autoencoder}
% \centering
% \end{figure}

Our autoencoder is trained to minimise the loss function

\begin{equation}
\label{eqn:loss_function}
    \mathcal L(\mathbf x)= \underbrace{||\mathbf{x}- \mathbf{\hat x}||_2^2}_{\text{Reconstruction loss}} + \underbrace{\alpha ||\mathbf{c}||_1}_{\text{Sparsity loss}}
\end{equation}

where $\alpha$ is a hyperparameter controlling the sparsity of the reconstruction. The $\ell^1$ loss term on $\mathbf c$ encourages our reconstruction to be a sparse linear combination of the dictionary features. It can be shown empirically \citep{sharkey2023technical} and theoretically \citep{wright2022high} that reconstruction with an $\ell^1$ penalty can recover the ground-truth features that generated the data. For the further details of our training process, see Appendix \ref{appendix:hparam_selection}.



==> neurips_workshop/further_autointerpretability_results_neurips.tex <==
\subsection{Interpretability is Consistent across Dictionary Sizes}

We find that larger interpretability scores of our feature dictionaries are not limited to overcomplete dictionaries (where the ratio, $R$, of dictionary features to model dimensions is $>1$), but occurs even in dictionaries that are smaller than the underlying basis, as shown in Figure \ref{fig:dictionary_size_comparison}. These small dictionaries are able to reconstruct the activation vectors less accurately, so with each feature being similarly interpretable, the larger dictionaries will be able to explain more of the overall variance.

\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]
    {images/interp_across_ratio.png}
    \caption{Comparison of average interpretability scores across dictionary sizes. All dictionaries were trained on 20M activation vectors obtained by running Pythia-70M over the Pile with $\alpha=.00086$.}
    \label{fig:dictionary_size_comparison}
\end{figure}


\subsection{High Interpretability Scores Are Not an Artefact of Top Scoring}

A possible concern is that the autointerpretability method described in Section \ref{section:autointerp} combines top activating fragments (which are usually large) with random activations (which are usually small), making it relatively easy to identify activations. Following the lead of \citet{bills2023language}, we control for this by recomputing the autointerpretation scores by modifying Step 3 using only randomly selected fragments. With large sample sizes, using random fragments should be the true test of our ability to interpret a potential feature. However, the features we are considering are heavy-tailed, so with limited sample sizes, we should expect random samples to underestimate the true correlation.

In Figure \ref{fig:residual_random_activations} we show autointerpretability scores for fragments using only random fragments. Matching \citet{bills2023language}, we find that random-only scores are significantly smaller than top-and-random scores, but also that our learned features still consistently outperform the baselines, especially in the early layers. Since our learned features are more sparse than the baselines and thus, activate less on a given fragment, this is likely to underestimate the performance of sparse coding relative to baselines.

An additional potential concern is that the structure of the autoencoders allows them to be sensitive to less than a full direction in the activation space, resulting in an unfair comparison. We show in Appendix \ref{appendix:topk} that this is not the source of the improved performance of sparse coding.

% We can further show that our larger interpretability score are an artifact of mixing not the source of the higher interpretability of sparse coding by looking at 'top-only' interpretability scores which looks at correlations in fragments with maximum activations.

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]    {images/residual_random_means_and_cis_new.png}
    \caption{Random-only interpretability scores across each layer, a measure of how well the interpretation of the top activating cluster is able to explain the entire range of activations.}
    \label{fig:residual_random_activations}
\end{figure}

While the residual stream can usually be treated as a vector space with no privileged basis (a basis in which we would expect changes to be unusually meaningful, such as the standard basis after a non-linearity in an MLP), it has been noted that there is a tendency for transformers to store information in the residual stream basis\citep{dettmers2022llm}, which is believed to be caused by the Adam optimiser saving gradients with finite precision in the residual basis\citep{elhage2023privileged}. We do not find residual stream basis directions to be any more interpretable than random directions.


\subsection{Interpreting the MLP Sublayer}

Our approach of learning a feature dictionary and interpreting the resulting features can, in principle, be applied to any set of internal activations of a language model, not just the residual stream. Applying our approach to the MLP sublayer of a transformer resulted in mixed success. Our approach still finds many features that are more interpretable than the neurons. However, our architecture also learns many dead features, which never activate across the entire corpus. In some cases, there are so many dead features that the set of living features does not form an overcomplete basis. For example, in a dictionary with twice as many features as neurons, less than half might be active enough to perform automatic interpretability. The exceptions to this are the early layers, where a large fraction of them are active. 

For learning features in MLP layers, we find that we retain a larger number of features if we use a different matrix for the encoder and decoder, so that the equations for our output $\hat x$ become

\begin{eqnarray}
\mathbf{c} &=& ReLU(M_e\mathbf{x}+\mathbf{b}) \label{eq:untied_encoder}\\
\mathbf{\hat x} &=& M_d^T \mathbf{c} \label{eq:untied_decoder}
\end{eqnarray}

\begin{figure}
    \label{fig:topk_mlp}
    \centering
    \includegraphics[width=.9\textwidth]{images/combomlp.png}
    \caption{Top-and-random and random-only interpretability scores for across each MLP layer, using an $\ell^1$ coefficient $\alpha=3.2e-4$ and dictionary size ratio $R=1$.}
\end{figure}


We are currently working on methods to overcome this and find truly overcomplete bases in the middle and later MLP layers.

\subsection{Interpretability Scores Correlate with Kurtosis and Skew of Activation}

It has been shown that the search for sparse, overcomplete dictionaries can be reformulated in terms of the search for directions that maximise the $\ell^4$-norm \citep{qu2019analysis}.

We offer a test of the utility of this by analysing the correlation between interpretability and a number of properties of learned directions. We find that there is a correlation of 0.19 and 0.24 between the degree of positive skew and kurtosis respectively that feature activations have and their top-and-random interpretability scores, as shown in Table \ref{tab:moment_correlation}.

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|}
        \hline
        \textbf{Moment} & \textbf{Correlation with top-random interpretability score} \\
        \hline
        Mean & -0.09\\
        \hline
        Variance & 0.02 \\
        \hline
        Skew & 0.20 \\
        \hline
        Kurtosis & 0.15 \\
        \hline
    \end{tabular}
    \caption{Correlation of interpretability score with feature moments across residual stream results, all layers, with dictionary size ratios $R \in \{0.5, 1, 2, 4, 8\}$.}
    \label{tab:moment_correlation}
\end{table}

This also accords with the intuitive explanation that the degree of interference due to other active features will be roughly normally distributed by the central limit theorem. If this is the case, then features will be notable for their heavy-tailedness.

This also explains why Independent Component Analysis (ICA), which maximises the non-Gaussianity of the found components, is the best performing of the alternatives that we considered.


==> neurips_workshop/introduction_neurips.tex <==
Advances in artificial intelligence (AI) have resulted in the development of highly capable AI systems that make decisions for reasons we do not understand. This has caused concern that AI systems that we cannot trust are being widely deployed in the economy and in our lives, introducing a number of novel risks \citep{hendrycks2023overview}, including potential future risks that AIs might deceive humans in order to accomplish undesirable goals \citep{ngo2022alignment}. Mechanistic interpretability seeks to mitigate such risks through understanding how neural networks calculate their outputs, allowing us to reverse engineer parts of their internal processes and make targeted changes to them \citep{cammarata2021curve, wang2022interpretability, elhage2021mathematical}.

To reverse engineer a neural network, it is necessary to break it down into smaller units (features) that can be analysed in isolation. Using individual neurons as these units has had some success \citep{olah2020zoom, bills2023language}, but a key challenge has been that neurons are often \textit{polysemantic}, activating for several unrelated types of feature \citep{olah2020zoom}. Also, for some types of network activations, such as the residual stream of a transformer, there is little reason to expect features to align with the neuron basis \citep{elhage2023privileged}.

\citet{elhage2022toy} investigate why polysemanticity might arise and hypothesise that it may result from models learning more distinct features than there are dimensions in the layer. They call this phenomenon \textit{superposition}. Since a vector space can only have as many orthogonal vectors as it has dimensions, this means the network would learn an overcomplete basis of non-orthogonal features. Features must be sufficiently sparsely activating for superposition to arise because, without high sparsity, interference between non-orthogonal features prevents any performance gain from superposition. This suggests that we may be able to recover the network's features by finding a set of directions in activation space such that each activation vector can be reconstructed from a sparse linear combinations of these directions. This is equivalent to the well-known problem of sparse dictionary learning  \citep{olshausen1997sparse}. 

% Building on \citet{sharkey2023technical}, we train sparse autoencoders to learn these sets of directions. Our approach is also similar to \citet{yun2021transformer}, who apply sparse dictionary learning to all residual stream layers in a language model simultaneously, and forthcoming work by Anthropic, who apply this method to a custom 1-layer transformer \citep{anthropic2023}. Our method is summarised in Figure \ref{fig:overview} and described in Section \ref{section:dictionary_learning}.

Building on \citet{sharkey2023technical}, we train sparse autoencoders to learn these sets of directions. Our approach is also similar to \citet{yun2021transformer}, who apply sparse dictionary learning to all residual stream layers in a language model simultaneously. Our method is summarised in Figure \ref{fig:overview} and described in Section \ref{section:dictionary_learning}.

We then use several techniques to verify that our learned features represent a semantically meaningful decomposition of the activation space. First, we show that our features are on average more interpretable than neurons and other matrix decomposition techniques, as measured by autointerpretability scores (Section \ref{section:autointerp}) \citep{bills2023language}. We then run case studies on a small number of features, showing that they are not only monosemantic but also have predictable effects on the model outputs, and can be used for fine-grained circuit detection. (Section \ref{section:monosemantic}).

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{images/sparse_coding_overview_1309.png}
    \caption{An overview of our method. We a) sample the internal activations of a language model, either the residual stream, MLP sublayer, or attention head sublayer; b) use these activations to train a neural network, a sparse autoencoder whose weights form a feature dictionary; c) interpret the resulting features with techniques such as OpenAI's autointerpretability scores.}
    \label{fig:overview}
\end{figure}


==> neurips_workshop/neurips_conclusion.tex <==
\subsection{Related Work}

A limited number of previous works have learned dictionaries of sparsely-activating features in pre-trained models, including \citet{yun2021transformer} and \citet{sharkey2023technical}, the latter of which motivated this work. However, similar methods have been applied in other domains, in particular in understanding neurons in the visual cortex \citep{olshausen2004sparse, wright2022high}. 

In contrast to our approach, where we try to impose sparsity after training, many previous works have encouraged sparsity in neural networks via changes to the architecture or training process. These approaches include altering the attention mechanism \citep{correia2019adaptively}, adding $\ell^1$ penalties to neuron activations \citep{kasioumis2021elite, georgiadis2019accelerating}, pruning neurons \citep{frankle2018lottery}, and using the softmax function as the non-linearity in the MLP layers \citep{elhage2022solu}. However, training a state-of-the-art foundation model with these additional constraints is difficult \citep{elhage2022solu}, and improvements to interpretability are not always realized \citep{Meister2021IsSA}.

\subsection{Conclusion}

Sparse autoencoders are a scalable, unsupervised approach to disentangling language model network features from superposition. Our approach requires only unlabelled model activations and uses orders of magnitude less compute than the training of the original models. We have demonstrated that the dictionary features we learn are more interpretable by autointerpretation and are more monosemantic than comparable methods. This approach could facilitate the mapping of model circuits, targeted model editing, and a better understanding of model representations.


==> sections/aidan_concept_editing_results.tex <==
\iffalse

``By ablating select features in these dictionaries, we can remove
model capabilities such as pronoun prediction, while disrupting model behaviour less than contemporary techniques.''

High level scratch work:
iterate over dictionary, measure which ones (when ablated) reduce performance the most, ablate those directions, measure KL divergence of model over pile

Done on tasks: 
pronoun prediction task
tried this on IOI under a different metric (but probably an appendix)

Similar Papers:
LEACE
papers they cite


Section outline:
Background on concept erasure/leace
Explain the pronoun prediction task
Explain dataset
What it means to ablate
Description of our process
Show results via graphics


Q: What were the interpretations of the 10 features that we ablate?

\fi

\begin{figure}[ht]
    \centering
    
    \includegraphics[width=.8\textwidth]{images/aidan/erasure_across_depth_410m_gender.png}
    \caption{Comparison of concept erasure methods applied to Pythia-410M at various layers. We show the mean edit magnitude (top) and the ability of the altered model to complete the pronoun-prediction task (bottom). Lower is better in both plots. The horizontal `Base Perf.' line shows the performance of the unedited model, and the horizontal `Majority' line shows the accuracy of random guessing.}
    \label{fig:erasure_across_depth_gender}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=.8\textwidth]{images/aidan/erasure_across_depth_410m_pronoun.png}
    \caption{We find that the erasure ability of dictionary feature projections outperform LEACE and difference-in-means projections when transferred to a related task, both in terms of erasure precision as measured by mean edit magnitude (top) and their ability to harm model performance on the task (bottom). Lower is better in both plots.} %While not all dictionary features generalise, we note that the optimal features are in the top-four best-performing features on the first task (Appendix \ref{appendix:concept_erasure_transfer}).
    \label{fig:erasure_across_depth_pronoun}
\end{figure}

% Previous version:
% For further evidence of the interpretability of our dictionary features, we turn to \emph{concept erasure}. Concept erasure is the task of editing the internal representations of the model to remove a single model capability, as measured by reduced performance on a particular task, while aiming to minimally disrupt model behaviour \citep{belrose2023leace}.

To demonstrate that our dictionary features correspond to functional units in the network, we turn to \emph{concept erasure}. Concept erasure is the task of removing a specified feature from a learned representation \citep{belrose2023leace}. Here, we assess each variant of concept erasure by how much our edits hinder the ability of our models to predict a certain concept while aiming to otherwise minimally disrupt model behaviour. On this task, we are able to outperform methods such as LEACE \citep{belrose2023leace} that hide a concept from arbitrary linear probes, while still using single-rank ablations, which we claim is evidence that our linear features better represent the underlying computational units of the model.

\subsection{Erasure on the `Gender Prediction by Name' Task}

We evaluate our approach on the pronoun prediction task, using the `Gender by Name' dataset \citep{misc_gender_by_name_591}. In this task, we few-shot prompt Pythia-410M to complete sentences of the form ``My name is \emph{\{name\}} and my gender is \{\emph{gender}\}.'' with the stereotypical gender for a given name. We restrict ourselves to male and female genders for simplicity and measure language model predictive ability via the true positive rate of a classifier with log probabilities equal to the model output logits of the corresponding tokens.

The feature dictionaries we used were trained with $\ell^1$ penalty coefficient $\alpha=8e-4$ and dictionary ratio $R=4$. Note that in contrast to Pythia-70M, Pythia-410M has 24 layers and residual stream dimension $d_{\text{in}}=1024$. In this section, we perform \emph{full-rank ablations} of dictionary features by projecting model activations to the orthogonal complement of that feature. In other words, we prevent the model activations from activating in that direction.

% %original:
% To select dictionary features for ablation, we filter for the top four features in each layer which erase the most information about gender as learnable by a linear probe, and then rank by performance on a test dataset.

% %new:
To select dictionary features for ablation, we rank them by their ability to hide gender information from a linear probe, as in \citet{ravfogel2022linear}, and then evaluate the top four dictionary features on their performance at the `Gender by Name' task on a 32-element `train' dataset distinct from the test dataset.

We compare our approach to two benchmarks: LEACE \citep{belrose2023leace} and difference-in-means projections.
% \footnote{For difference-in-means projections, we apply the projection $\mathbf{x} - \mathbf{v}^T\mathbf{x} \cdot \mathbf{v}$, where $\mathbf{v}$ is the normalised difference-in-means vector $\mathbb{E}[\mathrm{Embed}(X) | \mathrm{male}] - \mathbb{E}[\mathrm{Embed}(X) | \mathrm{female}]$ where $\mathrm{Embed}(X)$ is the activation on datapoint $X$.}
The difference-in-means projection $P_\mathbf{u}$ is defined as

% \begin{align*}
%     \mathbf{v} = \mathbb{E}[\mathrm{Embed}(X) | \mathrm{male}] - \mathbb{E}[\mathrm{Embed}(X) | \mathrm{female}] \\
%     \hat{\mathbf{v}} = \frac{\mathbf{v}}{|\mathbf{v}|} \\
%     P_\mathbf{v}(\mathbf{x}) = \mathbf{x} - \hat{\mathbf{v}}^T \mathbf{x} \cdot \hat{\mathbf{v}}
% \end{align*}


\begin{eqnarray*}
    % \mathbf{v} &=& \sum_{X \in }\text{Embed}(X) \mid \text{male}] - \mathbb{E}[\text{Embed}(X) \mid \text{female}] \\
    \mathbf{u} &=& \frac{1}{|\mathcal M|}\sum_{\mathbf{v} \in  \mathcal M}\mathbf{v} - \frac{1}{|\mathcal F|}\sum_{\mathbf{w}\in \mathcal F}\mathbf{w}  \\
    \hat{\mathbf{u}} &=& \frac{\mathbf{u}}{\|\mathbf{u}\|} \\
    % P_{\mathbf{u}}(\mathbf{x}) &=& \mathbf{x} - \hat{\mathbf{u}}^\top \mathbf{x} \cdot \hat{\mathbf{u}} \\
    P_{\mathbf{u}}(\mathbf{x}) &=& \mathbf{x} - \langle \hat{\mathbf{u}}, \mathbf{x}\rangle \hat{\mathbf{u}}
\end{eqnarray*}


where $\mathcal M$ and $\mathcal F$ are the residual stream activations from the layer being studied corresponding to male and female prompts, respectively. In other words, difference-in-means projection finds the difference $\mathbf{u}$ between the centroids of each gender class, and projects each activation $\mathbf x$ onto the subspace orthogonal to that direction.

We apply erasure interventions to each layer individually, and we assume activations at different token positions are i.i.d. for the purposes of LEACE and difference-in-means projections.


We find single features in early layers of the model that, when ablated, outperform LEACE and difference-in-means projections in model prediction accuracy removal (Figures \ref{fig:erasure_across_depth_gender} and \ref{fig:erasure_across_depth_pronoun}) while having a lower disruption to model behaviour overall, as measured by KL-divergence on the training distribution (Appendix \ref{appendix:kl_div_pile}). % We also find that the features that prove most effective for edits have interpretable, token-level activations (Appendix \ref{appendix:concept-erasure-feature-interp}).

\subsection{Transfer to Pronoun Prediction}

In order to test for some limited generality in using our learned features for erasure, we test the ability for the features in the previous section to generalise to erasure on a different task. We instead few-shot prompt the model to perform completions of the form ``\{\emph{name}\} went to the store, where \{\emph{pronoun}\} bought an \{\emph{object}\}.'', choosing the stereotypical pronoun for a given name. We show in Figure \ref{fig:erasure_across_depth_pronoun} that the highest-ranked features for gender prediction often permit good erasure on the pronoun prediction task, while methods such as difference-in-means projection and LEACE fail.

==> sections/appendices/aidan_edit_mag.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=.8\textwidth]{images/aidan/feature_ident_curve_edit_l11.png}
%     \caption{We are able to steer the model to the same degree via patching as other decompositions at the same magnitude of intervention. We find that the magnitude of intervention versus steering amount Pareto frontier shifts to the left as the sparsity of the learned dictionary decomposition increases, albeit at the cost of a larger maximum steering amount.}
%     \label{fig:edit_mag_vs_steering}
% \end{figure}

% We found that as well as achieving steering in a smaller number of patches, we are also able to steer to a greater degree with a smaller edit (Figure \ref{fig:edit_mag_vs_steering}).

==> sections/appendices/aidan_erased_feature_interp.tex <==
\iffalse
%\subsection{Interpreting Intervened Features}

\label{appendix:concept-erasure-feature-interp}

We plot token activation histograms (see Section \ref{section:case_studies}) for the features we ablate in Section \ref{section:concept_erasure}. Note that pronoun-related tokens (such as `\_she', `\_her' etc) appear in the top-5 most commonly activated tokens for the first three layers' features.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/aidan/hist_0_1486_0.50.png}
    \includegraphics[width=0.5\textwidth]{images/aidan/hist_1_309_0.50.png}
    \includegraphics[width=0.5\textwidth]{images/aidan/hist_2_1374_0.50.png}
    
    \includegraphics[width=0.5\textwidth]{images/aidan/hist_3_855_0.57.png}
    \includegraphics[width=0.5\textwidth]{images/aidan/hist_4_1249_0.54.png}
    \caption{Histograms of token activations for the ablated directions in Section \ref{section:concept_erasure}.}
\end{figure}
\fi

% \subsection{KL-Divergence on Training Distribution}

\label{appendix:kl_div_pile}

We measure the disruption to model behaviour by calculating the KL-divergence of the ablated model from the base model on the first 10,000 sequences from the Pile dataset \citep{gao2020pile}. We find that erasing the relevant dictionary features causes significantly less KL-divergence than difference-in-means projection or LEACE (Figure \ref{fig:kl-across-depth}).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{images/aidan/kl_across_depth.png}
    \caption{KL-divergence of the ablated model from the base model on the Pile, versus the layer the concept erasure intervention is performed at. The last datapoint for the difference-in-means edit has been ommitted as it is multiple orders of magnitude larger than all other datapoints.}
    \label{fig:kl-across-depth}
\end{figure}

\iffalse

\subsection{Erasure on the Transfer Dataset}

While dictionary erasure methods do not always transfer to the secondary task, we find that the `correct' (most optimal) features for erasure are in the top-four best-performing features of the other dataset (Figure \ref{fig:transfer_optimum_perf}).

\fi

\iffalse
\subsection{Concept Erasure on Last Token}

\label{appendix:concept_erasure_last_position}

We perform the same concept erasure experiment as in Section \ref{section:concept_erasure}, restricting edits to the last token position and re-fitting the difference-in-means and LEACE projections (Figure \ref{fig:erasure_last_pos}). We note that here LEACE achieves perfect performance with minimal intervention, as our i.i.d. assumption is correct.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{images/aidan/erasure_across_depth_last_pos.png}
    \caption{Erasure via editing the last token position of the gender-prediction prompt.}
    \label{fig:erasure_last_pos}
\end{figure}
\fi

==> sections/appendices/aidan_number_of_features.tex <==
% As of 8/15 we're NOT planning for this to not be in the 8/18 draft. Omit for now

Aidan's work, describing what we did to estimate the number of features, including any figures, etc. 

==> sections/appendices/feature_MCS_results.tex <==
can use MCS to look at the similarity of the dictionaries, between dicts of the same layer/same hparams, same layer/diff hparams, diff layer/same hparams
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{images/mcs_place.png}
    \caption{Graphs showing MCS results}
    \label{fig:mcs_place}
\end{figure}

==> sections/appendices/outlier_dimensions.tex <==
Outlier dimensions are dimensions in the residual stream with extremely high values. For Pythia-70M, the top 3 dimensions have max-activating datapoints that are TODO standard deviations above the mean. They have caused problems when quantising language models \citep{dettmers2022llmint8}, and been studied before in a variety of models TODO cite


==> sections/introduction_old.tex <==
 %auto-ignore

% Aidan: maybe here put something like 'toy models of superposition proposes that the internal representations of neural networks trained on natural data are usefully represented as sparse linear combinations of features', and then 'under this assumption we can use blah blah to extract features'


Advances in artificial intelligence (AI) have resulted in the development of highly capable AI systems that make decisions for reasons we do not understand. This has caused concern that AI systems that we cannot trust are being widely deployed in the economy and in our lives, introducing a number of novel risks \citep{hendrycks2023overview}, including potential future risks that AIs might deceive humans in order to accomplish undesirable goals \citep{ngo2023alignment}. Mechanistic interpretability seeks to mitigate such risks through understanding how models calculate their outputs, allowing us to reverse engineer parts of their internal processes and make targeted changes to them \citep{christiano2021alignment, burns2022discovering, elhage2021mathematical}.
\blfootnote{Code to replicate experiments can be found at \url{https://github.com/HoagyC/sparse_coding}}

To understand a large model it is necessary to break the model down into smaller units which can be productively analysed in isolation. Using the individual neurons as these units has had some success \citep{olah2020zoom, bills2023language}, but a key challenge has been that these neurons are largely polysemantic - activating for many unrelated types of input. Also, for some model activation types (such as the residual stream of a transformer) there is little reason to expect the neurons to be a reasonable unit of analysis and massive polysemanticity is the norm.

Some recent work has attempted to solve polysemanticity by training models where it does not arise \citep{elhage2022solu}, but training fully monosemantic models is not thought to be possible \citep{anthropic2023}. Another approach focuses on specific network features that are hypothesized to exist and uses supervised probes to detect if and how the information is represented \citep{gurnee2023finding}. However, this is both difficult to scale and relies on knowing which features to expect.

\citet{elhage2022toy} investigate why polysemanticity exists and hypothesize that it is the result of models trying to represent more features than the dimension of the layer, which is made possible by the sparsity of those features in the input data. This suggests that 
Although there is uncertainty about how neural networks represent information in their internal activations, one hypothesis is that their representations are \emph{linear with superposition} \citep{elhage2021mathematical, elhage2022toy, yun2023transformer, gurnee2023finding}. This posits (1) linearity: directions in neural activation space correspond to human-understandable \textbf{network features}, and (2) superposition: that there are more network features than the layer dimension, and so network features are not all orthogonal; instead, they form an `overcomplete basis'. The linear with superposition hypothesis suggests that finding human-understandable explanations of neural networks' internal workings will involve identifying the directions that correspond to network features. We would like some method to identify these directions. 

The hypothesis that the directions form an overcomplete basis rules out the use of dimensionality reduction methods, such as Principal Component Analysis (PCA), Independent Component Analysis (ICA), or Non-negative Matrix Factorisation (NMF), since these methods are limited to finding a number of directions no higher than the dimensionality of the activation space. 

We instead build on \citet{taking_features_out_of_superposition}, who use unsupervised sparse dictionary learning \citep{olshausen1997sparse} to extract large numbers of features from the neural activations of language models. The approach is related to \citep{yun2023transformer}, who also use unsupervised dictionary learning on model activations over a text corpus to represent the model's internal activations as a sparse linear combination of neural activations (Section \ref{section:sparse_autoencoder}). Unlike Yun et al., we apply sparse coding to each layer separately, instead of to the whole residual stream and also apply it to the MLP activations. 


% Our approach, outlined in Figure \ref{fig:overview}, samples the internal activations of a language model over a text corpus, and trains an autoencoder to reconstruct these activations as a sparse linear combination of dictionary features. If we assume that network activations consist of sparse linear combinations of ground truth network features, the resulting \emph{feature dictionary} (i.e., the weight matrix of the autoencoder) should learn dictionary features that are the same direction as the ground truth network features. We can therefore attempt to interpret the dictionary features in an attempt to understand the network.


\begin{figure}
    \label{fig:overview}
    \centering
    \includegraphics[width=1\textwidth]{images/sparse_coding_overview_1309.png}
    \caption{An overview of our method. We a) sample the internal activations of a language model, either the residual stream, MLP sublayer, or attention head sublayer; b) use these activations to train a neural network, a sparse autoencoder whose weights form a feature dictionary; c) interpret the resulting features with techniques such as OpenAI's autointerpretability scores.}
\end{figure}

Our features are learned without any reference to the meaning of the text, so we use several techniques to verify that our features are semantically meaningful and human-interpretable. First, we show that our features are, on average, more interpretable than other techniques as measured by autointerpretability scores \citep{bills2023language}. Next, we show that our features enable less-disruptive model concept erasure (Section \ref{section:concept_erasure}). We also show that we are able to pinpoint causally-important features for a set task (Section \ref{section:identifying_causal_features}). Finally, we provide evidence that our features are monosemantic across their activation range (Section \ref{section:monosemantic}). 

==> sections/related_work.tex <==
The desire to be able to interpret models is a common one and there have been a lot of approaches to doing this. A number of works have 
Prior work on learning dictionaries of activations is limited, with  \citet{yun2023transformer} being the most direct precusor work, but there have been a number of works which try to embed interpretability into the model itself through various forms of sparsity. This can be through altering the attention mechanism (adaptively sparse transformers), pruning neurons (lottery ticket) , adding l0 or l1 penalties to neurons (Elite Backprop - L1 above a threshold number) or (accelerating convolutional neural networks, l1 general, solu).
However, these models were generally trained on small datasets and even then there's often a noticeable hit to performance, and training a state-of-the-art foundation model with these is difficult,

